The Reverse Quantum Limit: Implications for Unconventional Quantum Oscillations in YbB$_{12}$

Beyond the quantum limit, many-body effects are expected to induce unusual electronic phase transitions. Materials possessing metallic ground states with strong interactions between localized and itinerant electronic states are natural candidates for the realization of such quantum phases. However, the electronic correlations responsible for increasing the likelihood of novel phases simultaneously place the quantum limit beyond the reach of laboratory magnets. Here we propose these difficulties can be surmounted in materials with strong correlations and insulating ground states. Strong correlations in insulators and high magnetic fields conspire to fill Landau levels in the reverse order compared to conventional metals, such that the lowest Landau level is the first observed. Consequently, the quantum limit in strongly correlated insulators is reached in reverse and at fields accessible in laboratories. Quantum oscillations measured at high fields in YbB12 are shown to have features consistent with the reverse quantum limit. These include how quantum oscillations move in lock step with the angular evolution of the insulator-metal transition and the field dependence of the quantum oscillation frequency. We argue that close to the insulator-metal transition, the insulating state should be viewed through the lens of a magnetic field-induced electronic instability affecting the lowest Landau level states in the quantum limit.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


